Enabling Uniform Computer Interaction Experience for Blind Users through Large Language Models

Blind individuals, who by necessity depend on screen readers to interact with computers, face considerable challenges in navigating the diverse and complex graphical user interfaces of different computer applications. The heterogeneity of various application interfaces often requires blind users to remember different keyboard combinations and navigation methods to use each application effectively. To alleviate this significant interaction burden imposed by heterogeneous application interfaces, we present Savant, a novel assistive technology powered by large language models (LLMs) that allows blind screen reader users to interact uniformly with any application interface through natural language. Novelly, Savant can automate a series of tedious screen reader actions on the control elements of the application when prompted by a natural language command from the user. These commands can be flexible in the sense that the user is not strictly required to specify the exact names of the control elements in the command. A user study evaluation of Savant with 11 blind participants demonstrated significant improvements in interaction efficiency and usability compared to current practices.

==> Alt-Text/Alt-Text.tex <==
Fig. 1: A diagram showing the LLM-powered automation of a series of screen reader actions initiated by the user's natural language command within a Word document.

Fig. 2: A flowchart illustrating the architecture of the Savant system. In the figure, CE stands for Control Element, Value (CE) stands for the value of the Control Element, and NLC stands for Natural Language Command.

Fig. 3: Box plots displaying quantitative data collected from the user study.

Table 1: Demographic details of participants in the user study.

Table 2: A list of tasks that participants were required to complete during the user study. Depth represents the number of user interactions needed to
navigate from the root to a specific element to complete the task.

Table 3: Demographic information of participants in the Wizard-of-Oz study. GA refers to Google Assistant. All data is self-reported.

Table 4: Tasks assigned to participants in the Wizard-of-Oz study.

Author details:

Satwik Ram Kodandaram 
Utku Uckun - This research was done while this author was at Stony Brook University.
Xiaojun Bi
IV Ramakrishnan
Vikas Ashok
Note: Authors 1 and 2 contributed equally to this research.

==> Sections/3.PreliminaryStudy.tex <==
\definecolor{Gray}{gray}{0.85}
% \newcolumntype{p}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\section{Preliminary Study}

Since there currently exists no system capable of interpreting natural language requests for desktop interaction, we conducted an IRB-approved Wizard-of-Oz study with $11$ screen reader users using a standard screen reader keyboard shortcut and a make-believe voice-activated desktop interface operated by a ``wizard'' – a human operator simulating the intelligence of the system.

As mentioned earlier, the main goal of the study is to understand the user requirements and gain insight into how people with visual impairments use different variations of natural language queries to interact with desktop applications to perform tasks. 

\subsection{Participants}

We recruited $11$ ($P1$ to $P11$) screen reader users for our study. The average age was $52.5$ (median=$58$, SD=$15.1$, range=$31$-$73$). Gender representation was almost equal, with $6$ Female and $5$ male participants. Recruitment was done using an email list with simple random sampling. Inclusion criteria for the study were: (i) exclusive dependence on a screen reader with no functional vision, (ii) proficiency with \textit{JAWS} screen reader software, and (iii) familiarity with \textit{Windows} operating system platform and desktop applications. 

Participants were asked about their voice assistant usage habits during a pre-study interview. Almost all of the participants ($10$) mentioned that they used voice assistant systems at least once a day. $P2$ said he uses them at least once a week. $8$ participants mentioned that they use use Siri~\cite{Siri}, $9$ participants mentioned Amazon Alexa~\cite{Alexa}, and $4$ participants said they use Google Assistant~\cite{Google-Assistant}. Some common use cases for voice assistants were setting up alarms/timers/reminders, dictating messages and emails, making phone calls, or querying information such as weather, traffic, or trivia. More details about participant demographics and their voice assistant usage habits can be found in Table \ref{tab:voice-study-participant}.

\begin{table*}[t]
    \begin{adjustbox}{center}
    \captionsetup{justification=centering}
    \centering
     \begin{tabular}{|c|c|c|c|c|c|}
        \hline
         \textbf{ID} & \textbf{Gender} & \textbf{Age} & \textbf{Acuity} &\textbf{Voice Assistant}& \textbf{Use Cases}\\ \hline
         \textbf{P1} & Male & $40$ & No vision & Alexa and Siri & Calendar, Email, Messages, and Reminder \\ \hline
         \textbf{P2} & Male & $58$ & No vision & GA & Calls, Email, and Messages \\ \hline 
         \textbf{P3} & Female & $64$ & Light perception & Alexa and Siri & Info Query and Timers \\ \hline
         \textbf{P4} & Female & $61$ & No vision & Siri & Alarms, Calls, Email, Info Query, and Messaging \\ \hline
         \textbf{P5} & Female & $39$ & No vision & Alexa, GA, and Siri & Calculation, Games, and Info Query \\ \hline
         \textbf{P6} & Female & $35$ & Light perception & Alexa and Siri & Alarms, Calling, Emails,  Start Apps, and Timers \\ \hline
         \textbf{P7} & Male & $43$ & Light perception & Alexa, GA, and Siri & App Navigation, Info Query, and Online Shopping \\ \hline
         \textbf{P8} & Male & $71$ & No vision & Alexa and Siri & Calls, Calculation, and Contacts \\ \hline
         \textbf{P9} & Female & $73$ & No vision & Alexa & Calculations and Info Query \\ \hline
         \textbf{P10} & Male & $62$ & Light perception & Alexa and GA & Alarms, Online Shopping, Smart Home, and Timers \\ \hline
         \textbf{P11} & Female & $31$ & Light perception & Alexa and Siri & Calls, Info Query, Online Shopping, and Timers \\ \hline
    \end{tabular}
    \end{adjustbox}
    \setlength{\abovecaptionskip}{10pt}
    \caption{Preliminary study participant demographics. GA stands for Google Assistant. All information was self-reported.}
    \label{tab:voice-study-participant}
\end{table*}

\subsection{Study Design}

We conducted a user study using Wizard-of-Oz methodology to collect an initial dataset of natural language queries used by blind screen reader users. This methodology is commonly used before building dialog assistant systems~\cite{ashok2014dialogue}. Unknown to the participants, the experimenter controlled the voice assistant system and carried out their natural language queries. During the study, participants were given tasks from $5$ applications: Excel, File Explorer, Gmail, Word, and Zoom. These tasks can be found in Table~\ref{tab:voice_study_tasks}. In total, there were $26$ tasks to complete. The selection of these tasks was based on the key findings of the interview study in~\cite{uckun2022taming}, and these tasks are comparable in difficulty and capture the diversity in UI interactions for screen reader users. For each participant, the tasks were randomly split among the following three conditions, with at least three tasks per condition:

\begin{enumerate}
    \item \textbf{Keyboard only} – Tasks under this condition had to be completed using standard screen reader shortcuts, such as those available in JAWS.
    
    \item \textbf{Voice only} – Tasks placed in this condition had to be performed using natural language queries alone.

    \item \textbf{Combination} – In this condition, users could use voice and/or screen reader shortcuts at their discretion.

\end{enumerate}

\begin{table}[t]
    \begin{adjustbox}{center}
    \captionsetup{justification=centering}
    \centering
    \begin{tabular}{|c|c|}
    \hline
         \textbf{Application}& \textbf{Task} \\ \hline
         Excel & Add a sum function to this cell \\ \hline
         Excel & Freeze the top row \\ \hline
         Excel & Change the format of this number to fraction \\ \hline
         Excel & Highlight the selected cell yellow \\ \hline
         File Explorer & Move dog picture to photos folder \\ \hline
         File Explorer & Create a new folder named ``Tasks''\\ \hline
         File Explorer & Sort files in folder \\ \hline
         File Explorer & Select all files \\ \hline
         File Explorer & Share selected files \\ \hline
         File Explorer & Open file with Adobe Acrobat \\ \hline
         Gmail & Find the email from Google \\ \hline
         Gmail & Move email to promotions folder \\ \hline
         Gmail & Go to starred emails folder \\ \hline
         Gmail & Reply to email saying ``Thank you'' \\ \hline
         Gmail & Refresh your inbox \\ \hline
         Word & Grow font size to $14$ \\ \hline
         Word & Make text bold \\ \hline
         Word & Center the text \\ \hline
         Word & Undo action \\ \hline
         Word & Switch style to heading $1$ \\ \hline
         Word & Add a comment saying "change later" \\ \hline
         Word & Insert a table with $2$ rows and $3 $columns \\ \hline
         Zoom & start a new meeting with video off \\ \hline
         Zoom & Copy the invitation link to the meeting \\ \hline
         Zoom & Schedule a meeting for tomorrow $1$ PM \\ \hline
         Zoom & Message your contact Alex saying ``Hello'' \\ \hline
    \end{tabular}
    \end{adjustbox}
    \setlength{\abovecaptionskip}{10pt}
    \caption{Tasks given to the participants in the preliminary study.}
    \label{tab:voice_study_tasks}
\end{table}

\subsection{Measurement}

Audio recordings of the participants were collected during the study. These recordings were transcribed, and the participants' natural language queries for each task were collected. Time for task completion was also collected.

\subsection{Procedure}

The experimenter first explained to the participants that the goal of the study was to understand and collect the variations of natural language queries used to perform the task. The study was set up in a way that made it hard for them to discern that they were interacting with the wizard rather than the system. The experiment was conducted using a \textit{Windows} laptop with a JAWS screen reader. During the study, the users leaned forward as if to speak into the microphone and only turned toward the experimenter when they had questions. Finally, many users expressed interest in getting a copy of the system for testing as soon as possible, which also suggests that they preferred interacting with a functional voice-enabled interface.

Since voice-enabled interaction with the desktop applications was a new concept to all the participants, the experimenter provided a demonstration at the beginning of the experiment by performing a simple task and showing a wide range of voice commands that the participants could issue. After the demo session and collection of demographics data, participants were given $10$ minutes to practice their JAWS skills in the Word pad application. After the practice, participants were given another $10$ minutes to learn and get familiar with the voice-enabled user interface. After the practice and learning stages, participants completed tasks in $5$ applications using JAWS and \textit{\sysname{}} systems. The order of the applications was counterbalanced using the Latin square method~\cite{kim2009spreadsheet}. Lastly, participants were administered a custom questionnaire to collect subjective feedback. Each study lasted for nearly $2$ hours, and the participants were given monetary compensation for their time and contribution.

\subsection{Findings}

\paragraph{\textbf{Query Interface vs. Keyboard Shortcuts}}

Participants preferred to use the voice interface over the JAWS software in $231$ tasks out of $286$ ($\sim 81\%$). Participants $P1$, $P4$, $P5$, and $P6$ attempted to complete the keyboard-only tasks with JAWS but encountered difficulty and experienced frustration. As a result, they were permitted to use the voice interface, and they successfully completed the tasks.

\paragraph{\textbf{Task Completion Time}}

On average, it took $73.1$ seconds (median=$60$, SD=$52.9$) for participants to complete the various tasks using the JAWS screen reader. On the other hand, the voice interface took $30.2$ seconds (median=$20$, SD=$40.5$) on average. This finding endorses that a voice interface carrying out users' commands can drastically reduce the time they spend navigating the application and allow them to focus on the main goal.

\paragraph{\textbf{Patterns in Natural Language Queries}}

The first finding of our analysis was the participants' preference for composite queries over single-action queries. Some of the tasks in our study were multi-step tasks, meaning they can be completed either by giving a single \textit{composite} query or multiple single-action queries. For example, for moving the dog picture to the photos folder, a participant can either use the \textit{move} composite query or use \textit{Copy} and \textit{Paste} single-action queries. Out of $82$ natural language queries used in the multi-step tasks, $67$ were composite queries ($82\%$). This shows that participants prefer the interface to handle the intermediary actions rather than giving multiple queries.

Secondly, we examined how participants gave queries when the task required a target. We describe a target as the object the control will affect. For example, when highlighting a cell in Excel, the cell is the target of the \textit{highlight} action. For such tasks, participants can indicate the target by either using the keyboard to select it or include the target's name in the query they give (``Highlight the cell A1''). Out of $68$ queries that required a target, $23$ were indicated in the query ($34\%$). Even though this number is relatively small, it indicates that some participants would prefer the interface to be able to select the target.

\paragraph{\textbf{Variations in Natural Language Queries (NLQ)}}

All the \textit{NLQs} given by the blind screen reader users were collected during the study. It was found that blind screen reader users express different variations of \textit{NLQs} when performing a task. The user intention may not always accurately align with the variations in application controls. For instance, one of the tasks in \textit{Word} application required inserting a table with $2$ rows and $3$ columns. Most participants used the ``Create table'' command where \textit{Word} does not feature a distinct \textit{Create table} control.  Also, we identified many variations of how users can trigger a simple control. For example, the query ``Make the font size 12'', ``Increase the font size to 12'', and ``Make text size 12'' all respond to the same control (font size 12). This means the interface should be highly generalizable across applications/platforms and robust enough to comprehend the user's intention and map the application's accurate control. These \textit{NLQs} were analyzed for finding patterns and for use in developing and testing the query interface. 

\paragraph{\textbf{Subjective Feedback}}

All participants preferred using the query interface instead of JAWS keyboard shortcuts. Participants $P2$, $P4$, $P5$, $P8$, and $P11$ mentioned that using the query interface was much faster than trying to complete the tasks with JAWS. To quote participant $P8$, ``It was much faster than typing (using JAWS) ... you don't lose your chain of thought.'' Participants $P2$, $P3$, $P7$, $P9$, $P10$, and $P11$ stated that they loved interacting with computer applications without touching the keyboard. $P9$ said, ``It was less work than typing. No keystrokes, less memorization'' while $P7$ and $P10$ mentioned that the voice interface is necessary for people with motor disabilities or who cannot use their hands. 


==> ignore.tex <==
First,~\sysname{} will automatically extract all the GUI controls of any arbitrary application and generate a thorough non-visual representation of the GUI capturing all the application's controls, including \textit{Visible} (e.g., ribbon commands, user content, side-panels, menus), and Invisible (controls that are hidden behind other controls, e.g., sub-menus) controls, and their relationships (e.g., `parent of', `descendent of'). Then, using this non-visual representation of the GUI,~\sysname{} will generate an on-demand pop-up interface containing all the extracted application controls. The navigation inside the pop-up interface is \textit{Uniform}, i.e., navigating and accessing the controls of applications using the same basic shortcuts, such as \textit{ARROW} keys, \textit{TAB}, and \textit{ENTER}, thus obviating the need to memorize a wide array of shortcuts to access the application controls. The pop-up interface will also have a search functionality for the application controls, which further reduces the time needed to access the desired control, eliminating the need for tedious manual exploration of application GUI via screen reader shortcuts.

For instance, to perform table insertion in \textit{Word}, users can just utter, ``Create a table with $2$ rows and $3$ columns'', and~\sysname{} will understand the user intent, i.e., \textit{Insert table}, automate the task by simulating a click on \textit{Insert tab} -> \textit{Insert table} -> \textit{Select $2$ rows and $3$ columns}, return the control to the user, and user can complete the task 


 For instance, to ``change the Font size'' in \textit{Word} application involves navigating \textit{linearly} through multiple menus and dialog boxes. They need to use keyboard shortcuts and arrow keys to access the \textit{Home} tab, navigate to the \textit{Font group}, open the \textit{Font dialog box}, locate the \textit{Font Size} control, adjust the size, and confirm the changes. 

%Illusration
For instance, to freeze the first row in \textit{Excel}, users can just utter, ``Freeze the first row'', and~\sysname{} will comprehend the user intent, i.e., \textit{Freeze} action, and automate the task by positioning the cursor on row $2$ or below. It then simulates a series of clicks: accessing the \textit{View} tab in the Excel ribbon at the top of the window, locating the \textit{Freeze Panes} option in the \textit{Window} group, clicking on the \textit{Freeze Panes} drop-down arrow, and it returns the drop-down menu controls to the user in a pop-up interface. With the limited drop-down options, users can easily navigate with basic keyboard shortcuts in the pop-up interface and select \textit{Freeze Top Row} from the options and complete the task seamlessly.

%Proxy interface
blind users could encounter challenges identifying the specific control needed to perform a task amidst the plethora of options presented. This can lead to confusion and ineffectual navigation of the interface. 

These tasks were identified as representative and ``potentially useful'' for people with vision impairments by our colleague, who is a desktop accessibility consultant.

Crawler
% Microsoft UI Automation framework provides access to the UI Automation tree, which contains information about the desktop application's controls visible on the screen. Furthermore, it provides an API to perform various actions on these controls programmatically (e.g., font family dropbox can be extended, ``Insert'' tab can be selected). However, it is limited to only visible controls. To solve this issue, we developed a crawler module that creates a map of the desktop application's interface. 
Usually, on web pages, all the elements can be accessed from the HTML DOM tree. However, the GUI tree of desktop applications will have only visible application controls. These invisible controls are not revealed in the GUI tree unless users select the controls.

Since the crawling application takes a long time, it must run before using~\sysname{} and save its result to a readable medium. Therefore, once the crawling is done, the internal representation of the application's interface is saved to a JSON file. During runtime~\sysname{}, the system detects the current application the user interacts with and loads the file from the repository.

\sysname{} uses the crawler module's output to infer the application's complete interface hierarchy. Having access to the invisible controls increases the capabilities of \sysname{} system substantially. For example, the user can search for the controls that are not visible on the application's interface. For example, the user can search ``Times New Roman'' using the \sysname{} keyboard interface, and even though the ``Times New Roman'' control is not currently visible on the application's interface, the crawler's output will tell us that the control resides under the ``Font Family'' dropbox. 

The language Understanding module detects the user's intent, namely the control they want to trigger using LLMs. The Dialog Policy and Response Option Generator sub-modules populate the popup interface with a ranked list of responses in order of relevance to the query.

We represent the controls as ($<$Control$>$, $<$Value$>$) apriori pairs. For example, font size $12$  is represented as (font size, $12$). On the other hand, the ``Bold'' button in the Wordpad application is (Bold, None) since it is a control that does not take any value. Calibri font in Microsoft Word becomes (font family, Calibri), and so on. These pairs for all the application controls have been created automatically from the output of our crawler module.

with the user's natural language query and the GPT-4 model outputs which button the user wants to trigger. 

To leverage GPT-3 for a given task, it has to be adapted to the specifics of the task. This is done by carefully selecting few-shot examples as part of the prompt. Since our task is to map the user's command to a button in the application, 

After the list of ($<$Control$>$, $<$Value$>$) pairs, the prompt has a few training examples (few shots) to teach the model the task at hand. A training example for our task consists of a command and the button that the command should map to. An example of a training example is in the following form: \newline

\begin{center}
    Text: Set text size to 12
    
    Answer: (font size, 12)
\end{center}

Since the length of the prompt is limited (typically to $3000$ words), training examples must be chosen carefully for the best results. After experimenting with different numbers of examples, we found that $5$ training examples are sufficient to teach the model the task without exceeding the prompt quota. To have the most accurate model, we built and tested $2$ approaches for choosing the training examples. 

In the first approach, training examples were manually crafted to teach the model the task. These training examples were application-agnostic; therefore, they can be used in each prompt without alteration. This approach will be referred to as the handcrafted approach from now on.

The second approach is more context-aware, and the training examples were selected with respect to the application in use and the command the user gave. To choose training examples similar to the user's voice query, we needed two things: (i) a metric for evaluating the similarity between the user's query and a training example and (ii) a dataset of training examples to choose from. For the similarity metric, we used the BERT sentence distance between the user's voice query and the NLP command of a training example. To have a large pool of candidate training examples, a method that can create an NLP utterance for a given command was needed. Collecting this data from screen reader users for tens of applications and hundreds of controls would be unrealistic. Instead, 

Many tasks, in reality, will have multiple similar tasks, or the same task can be done in a different way. For example, in the \textit{Notepad} application, when the user query is ``Remove the selected text,'' the possible controls they are looking for can be either \textit{delete button} or \textit{cut button}. Understanding the user intent and presenting the right application control is very important. To handle these situations, the LLM will first check if there are multiple similar controls that exist for the user's query. If present, then LLM will return all possible controls and this will be presented to the user. Users can select the desired control and perform the task. If there are no similar controls, our system will generate the sequence of actions and automate it for the users.


Discussion:

Unlike web applications with standardized HTML structures, desktop applications vary in their implementations and lack consistent accessibility features, complicating the task of programmatically locating and interacting with controls. Moreover, the multitude of UI frameworks used to build desktop applications further adds to the complexity, as each framework may have its own methods for defining and managing controls. Automation tools for desktop applications are less mature than web applications, offering limited capabilities and sometimes facing security restrictions.

Invisible
Our system will present all the application controls, including visible and invisible controls, in a pop-up interface where users can use a basic screen reader shortcut to access . 

Detect and extract all the visible and invisible controls of the application automatically using the custom \textit{crawler} module and create a GUI representation containing pertinent information such as parent-child relationships and other control attributes. Leveraging the previous work of Uckun et al.,~\cite{uckun2022taming},~\sysname{} classify the extracted application controls as either command controls (e.g., font dropbox in \textit{Word}, New Slide button in \textit{PowerPoint}, etc.) or non-command controls (e.g., structural controls such as panes and ribbons), or primary content area controls (e.g., cells in \textit{Excel} Table, files/folder in \textit{File Explorer}). The identified command controls are then sent to the layout design module, which generates a dynamic pop-up interface for displaying these controls to the user.

In the case of the keyboard interface, the user only needs to press the \textit{TAB} key to move through the list of commands within the popup interface. The interface also includes a search function to help the user locate the desired command quickly. When a user selects a command in the pop-up interface, the \textit{Action Relay} module initiates an automatic selection or click event on the command in the application's graphical user interface.  In the case of the natural-language voice interface, the dialog assistant module analyses the user's voice input, identifies the requested task or action, and returns the application control and desired action corresponding to the input user utterance. Using this interpretation, the \textit{Action Relay} module initiates an automatic sequence of selection or click events on the controls in the application's graphical user interface. Also, the interface is automatically closed, and the screen reader focus returns to the application's GUI (precisely the GUI element that was in focus when the user selected the special \sysname{} shortcut). This allows the user to resume without any delays. 

% for the \textit{Gen LLM}, which generates the accurate action corresponding to the user's NLC.

In the dynamic phase, when a user activates the interface by pressing \textit{CTRL + I} shortcut, the system begins to listen to the user's natural language commands. It then converts these spoken commands into written text and employs the BERT sentence similarity search method~\footnote{\url{https://huggingface.co/tasks/sentence-similarity}} to retrieve relevant few-shot examples from the existing~\controlvalue{} pair and their corresponding NLC few-shot examples dataset.

We curated the few-shot examples dataset comprising a triplet for each application control: the control element, its value, and the corresponding natural language command to execute an action on that control element. This allows the system to retrieve relevant few-shot examples for the \textit{Gen LLM} in run-time when a user gives any NLC on any application control. To achieve this, we employed a reverse engineering technique.


Currently, our interface extracts and accesses only visible and invisible controls of the application's main window. It won't access the controls of a sub-window (e.g., In Notepad, when we click ``Settings'' control, all the settings options are displayed in a separate sub-window.) or a pop-up window control (e.g., In Word, when we click on ``Insert''->``Hyperlink'', a pop-up window appears where we can enter the address and display text for the hyperlink.). These windows often appear unpredictably in response to user actions or system events, making it difficult to anticipate their appearance and the controls they contain. Extracting all application controls necessitates a deeper understanding and analysis of the intricate relationships between various pop-ups/sub-windows and the application's main window. This entails discerning which pop-up windows are associated with specific controls within the main window. Additionally, the complexity is heightened by scenarios where multiple control actions prompt the display of the same pop-up windows, further complicating the extraction process. Furthermore, controls within pop-up windows and sub-windows often exhibit context-sensitive behavior, where their visibility, accessibility, or functionality depends on the state of the parent application or user interactions. For instance, the toolbar options available might change based on whether the user is editing text, inserting a table, or formatting a picture. This dynamic behavior makes it challenging to extract and interact with controls programmatically.


% During the user study, one of the participants mentioned that they would like to have~\sysname{} in the \textit{mac} operating system. One of our limitations is that \sysname{} currently supports arbitrary desktop applications only in \textit{Windows} operating systems. Creating extensions to access all the controls in desktop applications on \textit{macOS} is challenging because it involves more engineering efforts as interacting with a highly intricate \textit{macOS} with a complex architecture, and its security measures are stringent to protect user data and system integrity. Moreover, frequent API changes across \textit{macOS} updates can render extensions incompatible. 

% Another limitation was that our interface supports only English language commands. Large language models (LLMs) can comprehend and convert non-English instructions into English. In the future, further investigation will be conducted to delve deeper into this matter since improvements in this area will significantly augment the accessibility to multi-lingual users. A third limitation is that our interface supports only application-level controls. Support of user-generated content inside the application has not yet been accomplished. 

% \fixmevk{$10$ is ridiculous! There is no difference between \sysname{}

% and \syscomp{}which doesn't match the previous metrics} 

The NLCs provided by the users proved to be somewhat intricate, leading to occasional difficulties for the LLM in generating accurate responses. Consequently, users often had to issue commands multiple times to get the desired outcome, which significantly extended the completion time. Additionally, errors in the speech-to-text conversion further exacerbated the situation, as the system failed to produce the correct response, necessitating users to redo the task. Complicating matters further, some commands were formulated with multiple instructions within a single command. For instance, when attempting to add a note in Excel, participants used the NLC: ``Select this cell and add a note.'' Unfortunately, the LLM struggled to interpret this complex command correctly.


When asked about their preferred system, all participants chose~\sysname{}. As a reason for their decision, participants $P1$, $P2$, $P3$, $P6$, and $P11$ mentioned Savant to be highly user-friendly. Quoting Participant P2 - ``I like the voice (~\sysname{}) because sometimes I feel lazy and using the voice is direct and easy.''. Participants $P4$, $P7$, $P8$, and $P9$ mentioned they liked that there were fewer keyboard presses and navigating to find the controls. To quote $P8$ - ``Less navigation, fewer keyboard presses makes everything faster''. $P6$ and $P9$ mentioned they like that ~\sysname{} has the same command interface for all the applications, which is a cool idea. P6 said, ``People (screen reader users) are used to Tab and Shift+Tab controls. Performing a task with only fewer familiar keys is much better''. Many participants said that our system should have an alternate pop-up interface like~\syscomp{}. Their reason was: ``It (keyboard interface) gives me more opportunities when I can't use my voice: in a silent place (library), in a Zoom meeting, when there are background noises''. 

% On average, participants rate JAWS condition $49.9$ (median=$45.8$, SD=$20.9$), ~\sysname{} without Speech condition $10.1$ (median=$5$, SD=$12.43$) and, ~\sysname{} condition $7.42$ (median=$2.83$, SD=$10.36$). A higher NASA-TLX score indicates participants had a more difficult time under the JAWS condition. Shapiro-Wilk test showed departure from normal distribution for ~\sysname{} without Speech (W=$0.78$, p=$0.005$) and ~\sysname{} (W=$0.73$, p=$0.001$). Wilcoxon Signed Rank test showed that improvements at NASA-TLX score under both ~\sysname{} without Speech (W=$0.0$, p=$0.003$) and ~\sysname{} (W=$0.0$, p=$0.003$) conditions over the JAWS condition were statistically significant. However, the Wilcoxon test among ~\sysname{} conditions shows that there was not a statistical significance between the conditions (W=$13.0$, p=$0.139$).
